Parallel Training of GRU Networks with a Multi-Grid Solver for Long Sequences

Parallelizing Gated Recurrent Unit (GRU) networks is a challenging task, as the training procedure of GRU is inherently sequential. Prior efforts to parallelize GRU have largely focused on conventional parallelization strategies such as data-parallel and model-parallel training algorithms. However, when the given sequences are very long, existing approaches are still inevitably performance limited in terms of training time. In this paper, we present a novel parallel training scheme (called parallel-in-time) for GRU based on a multigrid reduction in time (MGRIT) solver. MGRIT partitions a sequence into multiple shorter sub-sequences and trains the sub-sequences on different processors in parallel. The key to achieving speedup is a hierarchical correction of the hidden state to accelerate end-to-end communication in both the forward and backward propagation phases of gradient descent. Experimental results on the HMDB51 dataset, where each video is an image sequence, demonstrate that the new parallel training scheme achieves up to 6.5$\times$ speedup over a serial approach. As efficiency of our new parallelization strategy is associated with the sequence length, our parallel GRU algorithm achieves significant performance improvement as the sequence length increases.

==> sections/Related_Work.tex <==
\section{Related Work}
\label{sec:related_work}

In order to accelerate the training procedure of GRU, many previous efforts have largely focused on two parallelization strategies such as the \textit{data-parallelism} that distributes a batch of sequences over processors, and the \textit{model-parallelism} that distributes layers across multiple processors~\citep{ben2019demystifying,gunther2020layer}.

The primary strategy for parallelizing GRU is the data-parallelism inherent in mini-batch Stochastic Gradient Descent (SGD) \citep{you2019large,huang2013accelerating}.
However, the accuracy of mini-batch SGD degrades as the number of sequences in each mini-batch increases.
Moreover, although multiple mini-batches are processed in parallel, the training procedure of each sequence (within a mini-batch) is invariably sequential.
Alternatively, the GRU model can be parallelized across hidden layers~\citep{wu2016google,mxnet2018}.
This model-parallelism approach is beneficial when the network requires a large number of layers. However, in practice, a large-scale recurrent neural networks such as Google Neural Machine Translation (GNMT) developed by \citet{wu2016google} have 8 LSTM layers. Therefore, model-parallelism is difficult to achieve massive parallelism as the number of usable processors is limited to the number of layers.
A common problem in data-parallel and model-parallel algorithms for GRU is that they still suffer from the accuracy and training execution time when the length of sequence (i.e., the number of data samples in each sequence) is long.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.99\textwidth]{figures/parallelism/DP_MP_TP.pdf}
%     \caption{Parallel training algorithms for GRU}
%     \label{fig:parallelism}
% \end{figure}

% First of all, the training procedure of GRU is inherently sequential as GRU takes an entire sequences of data as input to capture any long-term dependency in the sequence.
% As the training procedure of GRU given each sequence is sequential, the primary strategy for parallelizing GRU is the data-parallelism.
% (Figure \ref{fig:parallelism}-(a))
% (Figure \ref{fig:parallelism}-(b))
% Similar to the other Deep Neural Network (DNN) models, the primary strategy for parallelizing GRU is the data-parallelism 
% As the GRU requires to take sequences of data as an input, 
% Hence, data-parallel training algorithm is still not beneficial for precisely capturing the long-range temporal dependency when the length of each sequence is extremely long.
% As shown in Figure \ref{fig:parallelism}-(b),


% \paragraph{Truncated Backpropagation Through Time for training RNN}
% Truncated backpropagation (Williams and Peng, 1990) is arguably the most practical method for training RNNs. The earliest use of truncated BPTT was by Elman (1990), and since then truncated-BPTT has successfully trained RNNs on word-level language modelling (Mikolov et al., 2010, 2011, 2009) that achieved considerable improvements over much larger N -gram models.
% \citet{sutskever2013training} 

% \paragraph{Deep Neural Network Multigrid Solver (DNN-MG)}
% \citet{hartmann2020neural,margenberg2020structure}

% \paragraph{ODE RNN}

==> sections/boneyard.tex <==
\section*{(Old) Parallel-in-Time Training}

Training GRU networks is typically done with the BPTT algorithm. This algorithm requires a forward evaluation of the neural network, followed by the adjoint or backpropagation to compute the gradient. Both forward and backward propagation are computationally expensive algorithms that don't naturally lend themselves to parallelization in the time domain. The proposed multigrid method avoids this issue by only approximately propagating through the neural network, essentially trading off accuracy for performance. This section motivates and develops the multigrid algorithm as applied to forward propagation. The backward propagation is essentially the same with the time evolution through the sequences reversed. We highlight notable differences within the text.



\subsection{A Parallel Method with Poor Algorithmic Performance}
Figure~\ref{fig:parallel-in-time} immediately suggests an approach to achieving time parallelism. Given $P$ independent processors, subdivide the time sequences accordingly, i.e. given $T_p = T/P$ each processor is assigned a sub-sequence of time step end points
\begin{equation}
\underbrace{t_1,\ldots, t_{T_p}}_{\text{Processor } 1}, \;
\underbrace{t_{T_P+1},\ldots, t_{2 T_p}}_{\text{Processor } 2}, \;
\ldots, \;
\underbrace{t_{(P-1)T_P+1},\ldots, t_{P T_p}}_{\text{Processor } P}.
\end{equation}
In this distribution, ownership of the time point implies that processor is responsible for computing the time step \emph{ending} at that time.

The parallel algorithm assumes an initial guess for the hidden state at all
the initial time points, denoted $h_t^0$ equal to zero. The initial guess for each state is distributed to the correct processor. Each processor then maps its initial states using the mapping in Eq.~\ref{eqn:gru-imap}, resulting in the new set of hidden states $h_t^1$. We further enforce that $h_0^1 = h_0^0$. Each processor, except the final, must communicate its last time evaluation to the processor immediately to its right. This process is repeated for $I$ iterations to achieve the hidden values $h_t^I$ at all the time steps.

The algorithm achieves parallelization by simultaneously computing the updates on each processor. In the limit of $P=T$, each time step evaluation is computed in parallel. In the algorithm described each time step is computed independently. A simple modification is to only maintain guesses at the boundaries between processors and use those to compute the hidden state at the last time value computed by that processor. This has a certain memory advantage but does not avoid the fundamental flaw in the algorithm.

The flaw is exposed by noting that the after one iteration, the values of $h_0$ and $h_1$ are correct (the first by construction using $h_0^0=0$, and the second because $h_1^1 = \Phi_1(x_1,h_0^0)$). This generalizes so that after $I$ iterations
we have $h_i=h_i^I$ for $i\leq I$. Thus to compute the hidden states
for all time steps requires $T$ iterations of the parallel algorithm with the cost of each iteration scaling with $T_p$, resulting in no speedup (and in this case a slowdown). The proposed modification fixes the slowdown, and requires only $P$ iterations, but the iteration cost scales with $T_p$ yielding a run time that scales with the number of time steps. While the poor algorithmic performance (requiring too many iterations) negates the benefit of the parallelization, this algorithm remains useful as the core parallel kernel in the development of our multigrid technique. Thus a variant of this algorithm, known as \FRelax is presented in Algorithm~\ref{alg:frelax}.

\subsection{A Coarse Initial Guess}


To improve the performance of the parallel algorithm, one approach is to improve the initial guess of the hidden state. A convenient choice, and
a computationally efficient one, is to use a coarser representation of the
sequence. Define, the coarse time nodes as
\begin{equation}
t_0, t_{c_f}, t_{2 c_f}, \ldots, t_{T_c c_f}
\end{equation}
where $T=T_c c_f$, $T_c$ is the length of the coarse sequence, and $c_f$ is the integral coarsening factor greater than $1$ $1$ (for convenience of notation assume $T$ is evenly divisible by $c_f$). 
A coarse representation of the original neural network can be defined as
\begin{equation}
\tilde{h}_{c_f t} = \Phi_{c_f}(x_{c_f t},\tilde{h}_{c_f(t-1)}) \quad \mbox{for }
t=1\ldots T_c.
\end{equation}
which provides an approximation of the hidden state on the fine level at the
coarse nodes
\begin{equation}
h_{c_f t} = \Phi_1(x_{c_f t},\Phi_1(x_{c_f t-1}, h_{c_f t -2})) \approx \tilde{h}_{c_f t}
\end{equation}

The challenge of accelerating propagation with parallelism arises from the need to communicate from the initial layer through to the final layer in a serial fashion. 
The algorithm proposed above defines an initial guess for the hidden state 
\begin{equation}
\Rfwd(h_0,h_1,\ldots h_T) = \left[h_t-\Phi_1(x_t,h_{t-1})\right]_{t=1}^T
\end{equation}


To resolve this, the multigrid-in-time algorithm efficiently communicates from end to end using a low-cost initial guess for the relaxation algorithm described above. The choice for the initial guess is to use a subsampling of the initial sequence, with a larger time step as required by the update algorithm in Eq.~\ref{eqn:gru-imap}. This is depicted visually in Figure~\ref{fig:mg-opt}, were the fine resolution (top row) of the sequence is used to construct coarser sequences with a sub-sampling rate (or coarsening factor) of $c_f=2$ in the picture.

\eric{Here I will talk through the multilevel algorithm}

Training GRU networks is typically done with the BPTT algorithm. This algorithm requires a forward evaluation of the neural network, followed by the adjoint or backpropagation to compute the gradient. The forward and adjoint systems for GRU can be written as a system of nonlinear equations using
\begin{multline}
\Rfwd(h_0,h_1,\ldots h_T) = \left[h_t-\Phi_1(x_t,h_{t-1})\right]_{t=1}^T \mbox{, and } \\
\Radj(\hat{h}_0,\hat{h}_1,\ldots \hat{h}_T) = \left[\hat{h}_{t-1}-\partial_h \Phi_1(x_t,h_{t-1})^T \hat{h}_t \right]_{t=1}^T 
\end{multline}
where $\hat{h}$ represents the adjoint variable. The serial forward and backpropagation algorithms determine the forward and adjoint states such that $\|\Rfwd(h_t)\| = \|\Radj(\hat{h}_t)\|=0$.
Considering this serial propagation there appears little possibility for introduction of time parallelism. However, this assumes that propagation is done exactly. Instead, the parallel-in-time algorithm inexactly solves for the states: e.g.  $\|\Rfwd(h_t)\| = \|\Radj(\hat{h})\|\leq \epsilon$, and is able to exploit enhanced parallelism as a result. The algorithm can bee repeated for multiple iterations until convergence is achieved. 

The solution procedure used is based on the multigrid-in-time (MGRIT) algorithm developed in~\cite{falgout2014parallel} and applied to NeuralODEs in~\cite{gunther2020layer,cyr2019multilevel}. Generically, multigrid methods have a long track history of delivering scalable solution methods for numerical PDEs. A complete discussion of the substantive theory, and variations is beyond the scope of this document. Here we present a minimal description for understanding the fundamentals of the method.

The MGRIT algorithm has been developed to solve numerical ODE's using the discrete propagator defined in Eq.~\ref{eqn:gru-implicit}. For the sake of simplicity assume that $T=c_f N - 1$. The integral $c_f$ is a coarsening factor that defines $N_c=N/c_f$ coarse time points $t_0,t_{c_f-1}, t_{2 c_f-1},\ldots, t_{N_c}$. Further the form of the propagator leads naturally to a coarse representation 
\begin{equation}
\Phi_{\Delta t}(x,h) = \Phi_{c_f \Delta t}(x,h) + O(\Delta t).
\end{equation}
This structure creates two RNN's, a \emph{fine} one evaluated on the original sequence and a relatively \emph{coarse} network evaluated on a sub-sampling of the original sequence. In this sense, the MGRIT algorithm creates a multi-level hierarchy of RNN's that share the same parameters. This idea is depicted schematically in
Figure~\ref{fig:mg-opt} using a sequence of movie frames. In this case three levels are shown, where the coarsening is defined from the level above.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/horse/horse.pdf}
    \caption{A description of a multi-level neural network hierarchy}
    \label{fig:mg-opt}
\end{figure}

\subsection{Relation to Truncated BPTT}
\cite{sutskever2013training}

\begin{enumerate}
    \item The gradient descent algorithm
    \item Inexactness in the time evolution
    \item Multi-level for forward and backward propagation (why implicit)
    \item discuss TBPTT
\end{enumerate}

\begin{algorithm}[t]
 $\{h_t'\}\gets \FRelax(\Delta t,c_f,\{x_t\},\{h_t\})$ \\
 \ParallelFor{$t_c \gets 1$ \KwTo $N/c_f$} {
  $t \gets t_c c_f$ \\
  $h_{t}' = \Phi_{\Delta t}(x_t,h_{t-1}') $
 }
 $\{h_t''\}\gets\FRelax(\Delta t,c_f,\{x_t\},\{h_t'\})$ \\
 \Return $\{h_t''\}$
\caption{$\mbox{FCFRelax}(\Delta t,c_f,\{x_t\},\{h_t\})$ - Fine-Coarse-Fine parallel relaxation}\label{alg:mg-opt}
\end{algorithm}

\begin{algorithm}[t]
 \SetKwFunction{FRelax}{FRelax}
 $\{h_t'\}\gets \FRelax(\Delta t,c_f,\{x_t\},\{h_t\})$ \\
 \ParallelFor{$t_c \gets 1$ \KwTo $N/c_f$} {
  $t \gets t_c c_f$ \\
  $h_{t}' = \Phi_{\Delta t}(x_t,h_{t-1}') $
 }
 $\{h_t''\}\gets\FRelax(\Delta t,c_f,\{x_t\},\{h_t'\})$ \\
 \Return $\{h_t''\}$
\caption{$\mbox{FCFRelax}(\Delta t,c_f,\{x_t\},\{h_t\})$ - Fine-Coarse-Fine parallel relaxation}\label{alg:mg-opt}
\end{algorithm}

==> tables/notations.tex <==
\begin{table*}[ht]
\centering
\caption{Notations for Recurrent Neural Networks}
\scalebox{0.85}{
\begin{tabular}{c||c}
Notation & Description                                         \\ \hline \hline
$M$        & Input vector size (each sample size) at time step $t$                \\ \hline
$K$        & Hidden units (\# of neurons in a hidden layer)  \\ \hline
$S$        & Total \# of sequences                           \\ \hline
$T$        & Each sequence length (\# of time steps in each sequence)                                \\ \hline
$\mathbf{h}_{t}$ $\in$ $\mathbb R^{K}$    & Hidden output at time step $t$ (for $t$ $=$ $0, ..., T-1$)          \\ \hline
$\mathbf{x}_{t}$ $\in$ $\mathbb R^{M}$    & Input vector at time step $t$ (for $t$ $=$ $0, ..., T-1$)           \\ \hline
$\mathbf{U}$ $\in$ $\mathbb R^{K \times M}$        & Weights (for connecting input to current hidden state at each time step)                           \\ \hline
$\mathbf{W}$ $\in$ $\mathbb R^{K \times K}$       & Weights (for connecting previous hidden output to current hidden state at each time step)                                              \\ \hline
$\mathbf{b}$ $\in$ $\mathbb R^{K}$        & Bias of neurons                                               \\ \hline
$B$        & Batch size (\# of sequences in each mini-batch) \\ \hline
\end{tabular}}
\end{table*}



% \begin{table*}[ht]
% \centering
% \caption{Notations for LSTM}
% \scalebox{1}{
% \begin{tabular}{c||c}
% Notation & Description                                         \\ \hline \hline
% $M$        & Input vector size (each sample size) at time step $t$                \\ \hline
% $K$        & Hidden units (\# of neurons in a hidden layer)  \\ \hline
% $S$        & Total \# of sequences                           \\ \hline
% $T$        & Each sequence length                                \\ \hline
% \textbf{h}$_{t}$ $\in$ $\mathbb R^{K \times 1}$    & Hidden output at time step $t$ ($\forall t$ $=$ $0, ..., T-1$)          \\ \hline
% \textbf{x}$_{t}$ $\in$ $\mathbb R^{M \times 1}$    & Input vector at time step $t$ ($\forall t$ $=$ $0, ..., T-1$)           \\ \hline
% \textbf{U} $\in$ $\mathbb R^{K \times K}$        & Recurrent inputs (rename?)                           \\ \hline
% \textbf{W} $\in$ $\mathbb R^{K \times M}$       & Weights (for connecting different components within each hidden layer at each time step)                                              \\ \hline
% \textbf{b} $\in$ $\mathbb R^{K \times 1}$        & Bias of neurons                                               \\ \hline
% $B$        & Batch size (\# of sequences in each mini-batch) \\ \hline
% \end{tabular}}
% \end{table*}
